Invariance Principle Meets Vicinal Risk Minimization

Deep learning models excel in computer vision tasks but often fail to generalize to out-of-distribution (OOD) domains. Invariant Risk Minimization (IRM) aims to address OOD generalization by learning domain-invariant features. However, IRM struggles with datasets exhibiting significant diversity shifts. While data augmentation methods like Mixup and Semantic Data Augmentation (SDA) enhance diversity, they risk over-augmentation and label instability. To address these challenges, we propose a domain-shared Semantic Data Augmentation (SDA) module, a novel implementation of Variance Risk Minimization (VRM) designed to enhance dataset diversity while maintaining label consistency. We further provide a Rademacher complexity analysis, establishing a tighter generalization error bound compared to baseline methods. Extensive evaluations on OOD benchmarks, including PACS, VLCS, OfficeHome, and TerraIncognita, demonstrate consistent performance improvements over state-of-the-art domain generalization methods.

==> sec/1_intro_copy.tex <==
\section{Introduction}
\label{sec:intro}

Deep learning demonstrated powerful capabilities in computer vision tasks~\cite{he2016deep, liu2020ms}.
However, deep models often perform poorly when applied to unseen domains~\cite{gulrajani2020search} because training deep models assume that the training and test sets are independently and identically distributed~\cite{sain1996nature}.
This assumption may broken in real-world applications that data distributions are dynamic and variable, known as out-of-distribution (OOD)~\cite{ahuja2021invariance}.
For instance, in medical image analysis, models are often trained on data from a single hospital due to privacy and security concerns. 
This limitation causes the model to underperform in other hospital data imaging from different devices or techniques~\cite{dgdr, liu2020ms}.
Arjovsky \etal~\cite{arjovsky2019invariant} noted that models mainly fail to generalize OOD because they capture spurious causal relationships in the training data.
Let's consider a classic example in domain generalization: the training set has "cows in the grass" and "camels in the sand," 
where the background takes up most of the content, which can easily lead to the model using the background as the main feature for classification, while our goal is to classify the animals.
While this also classifies the image into two categories, the model immediately misclassifies when a cow in the desert or a camel in the grass appears in the test set.
As shown in \cref{fig: ood_failed}, the background is the spurious feature, and the shape of the animal is the invariant feature.
The model captures false causality and uses the spurious feature as a classification criterion, resulting in a failure of generalization. 
This problem severely hampers the deployment of deep learning systems in real-world applications.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.35\textwidth]{./images/figure1.pdf}
  \caption{
  2D classification example illustrating domain generalization failed. 
  Blue makers are the training set, yellow makers are the test set, and triangles and circles denote different categories, respectively. 
  The dashed lines indicate generalization failure predictors.
 }
 \label{fig: ood_failed}
\end{figure}


\begin{figure*}[t]
  \centering
  \includegraphics[width=1\textwidth]{./images/figure2.pdf}
  \caption{
    (a) and (b) Example of generalized failure in 2D classification when features do not satisfy support overlap leading to model generalization failure;
    % (c) Example of successful generalization when sufficient support overlaps.
    (c)  Example of generalized success in 2D classification using semantic data augmentation to generate new samples enlarging support overlap.
 }
  \label{fig: overview} 
\end{figure*}

Invariant Risk Minimization (IRM)~\cite{arjovsky2019invariant} and its variants~\cite{krueger2021out, ahuja2021invariance, chang2020invariant} stand for one of the most representative methods for domain generalization (DG).
They compel models to learn features consistent across environments, avoiding spurious causal pitfalls introduce by empirical risk minimization (ERM)~\cite{sain1996nature}.
Although IRM appears promising intuitively, the practical outcomes present some unexpected challenges.
Ahuja \etal.~\cite{ahuja2021invariance} noted that for linear classification tasks, if features insufficiency support overlap, both ERM and IRM may fail to address the OOD problem.
Meanwhile, Elan \etal~\cite{rosenfeld2021the} point out IRM can fail catastrophically in non-linear regime unless the test data are sufficiently similar to the training distribution.
To understand the reasons for the generalization failure, Ye \etal~\cite{ye2022ood} quantifies the dataset in diversity and correlation dimensions and attempt to reveal the reasons for the generalization failure.
The results show that IRM and its variant algorithm (VREx) outperform ERM on datasets with large correlation shift. 
Unfortunately, the IRM series algorithms do not perform well on datasets with large diversity shift.
All of this evidence points to dataset diversity as the reason for the failure of IRM generalization.
Forexample, recalling the earlier example of "cows on grass" and "camels on sand", if we adding "cows on desert" to the training set, the model still risks falling into spurious causality. 
As shown in subfigure (a) of \cref{fig: overview}. 
Similarly, when there are "camels on grass" in the training set (subfigure (b) in \cref{fig: overview} shown  "cow on sand"), the model fails to generalize.


Other DG methods increase the diversity of dataset through data augmentation (DA)~\cite{yan2020improve, zhang_domain_2024}.
Mixup~\cite{zhang2017mixup} generated new data by mixing two samples, and the Mixup series method have been widely used for domain generalization~\cite{lee_decompose_2023, zhou2021domain}.
Forexample, MixStyle~\cite{zhou2021domain} generates new domain style samples by mixing the styles between different domains.
Lee \etal~\cite{lee_decompose_2023} applied the Mixup technique in the frequency domain to augment the shape features.
However, these methods still have limitation that mixing images from two classes does not necessarily result in enhanced samples belonging to them~\cite{concutmix}.

Recent work called semantic data augmentation (SDA) or feature augmentation has likewise made some progress in domain generalization~\cite{li_simple_nodate, wang2024inter}.
These methods perform semantic transformations by modifying features, such as the texture of the background or foreground, which not only increases diversity but is also computationally efficient ~\cite{bengio2013better, upchurch2017deep, ISDA}.
Li et al.~\cite{li_simple_nodate} add Gaussian noise to feature embeddings during training for DG.
Wang \etal~\cite{wang2024inter} proposed an SDA-based DG method to increase diversity between inter-classes and inter-domains.
The motivation behind these operations is deep features are typically linear~\cite{bengio2013better, upchurch2017deep}. 
Unfortunately, these methods suffer from the same problem as the Mixup series methods: over-augment may lead to label changing~\cite{zhu2024bayesian}.
Let's take an inappropriate but vivid example we cannot generate images of cows on Mars before Elon Musk makes it a reality. 
Additionaly, similar to mixup, the SDA method of generating new samples by changing features is also an implementation of VRM.

In summary, we advocate introducing the idea of VRM into the IRM algorithm increasing the diversity of datasets for domain generalization.
However, it is still a challenge to introduce VRM in IRM algorithm while enhancing the data to avoid label changes.
Recently, Bayesian random semantic data augmentation (BSDA)~\cite{zhu2024bayesian} try to address this issue. 
BSDA proposes a SDA strategy that includes semantic direction and semantic strength.
Similar to image transformation-based data augmentation (DA) methods, the semantic direction corresponds to the type of transformation applied, while the semantic magnitude represents the degree of that transformation.
To prevent label changing, BSDA employs variational inference to estimate the distribution of augmentable ranges, generating new sample points accordingly. 
However, BSDA has primarily been applied to medical image classification, and its efficacy in natural image classification and domain generalization remains unexplored. 

In this paper, we propose a new domain generalization algorithm, Bayesian Semantic Domain Generalization (BSDG), which incorporate the VRM idea into the IRM algorithm.
Specifically, We propose a domain shared semantic data augmentation module based on BSDA, allowing for the possibility of exchanging semantics between domain samples.
To avoid the model falling into spurious causal relationships, we use IRM as the learning framework.
Despite the simplicity of our method, our experiments demonstrate that incorporating BSDA effectively mitigates the generalization failure of IRM.
The main contributions of this paper are:
\begin{itemize}
  % \item We advocate introducing the idea of VRM into the IRM algorithm increasing the diversity of datasets for domain generalization.
  \item We propose a domain-shared semantic data augmentation module based on BSDA, allowing for the possibility of exchanging semantics between domain samples.
  \item We provide a theoretical analysis based on Rademacher Complexity, proving the generalization error upper bound of the model when BSDA is plugged.
  \item We conduct extensive experiments on challenging out-of-distribution (OOD) generalization benchmarks, including PACS~\cite{pacs}, VLCS~\cite{vlcs}, OfficeHome~\cite{officehome}, and TerraIncognita~\cite{beery2018recognition} datasets, demonstrating that our method outperforms competitive models.
\end{itemize}


==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\subsection{Domain Generalization}
Domain generalization aims to generalize effectively to unseen target domains by learning from one or more source domain datasets\cite{zhou2022domain}.
Existing DG methods include domain meta-learning\cite{li2018learning}, data augmentation (DA)\cite{yan2020improve, zhou2021domain}, decoupled representations\cite{bai2021decaug}, causal reasoning\cite{sun2016deep}, 
and invariant risk minimization (IRM) series \cite{arjovsky2019invariant, krueger2021out, chang2020invariant, ahuja2021invariance}.
This section introduces invariant risk minimization and methods based on data augmentation for DG.

\subsection{Invariant Risk Minimization}
Arjovsky \etal~\cite{arjovsky2019invariant} proposed the IRM framework to enhance model generalization by identifying invariant features across different domains. 
BIRM~\cite{lin2022birm} applies Bayesian estimation to mitigate overfitting risks in limited training environments by accounting for uncertainty in the data, further enhancing the model’s generalization capabilities.
However, the bi-level optimization problem in IRM is complex and computationally intractable in practical scenarios. 
Many subsequent works simplify IRM by introducing constraints to transform the bi-level optimization into a more feasible single-level problem~\cite{chen2022pair,ahuja2021invariance,lin2022birm}. 
For example, PAIR~\cite{chen2022pair} addresses by framing the problem as a multi-objective optimization to achieve Pareto-optimal solutions over ERM, IRMv1, and VREx penalties, yielding more robust generalization performance. 
IRM is also highly sensitive to risk variance across training domains, especially when there is a large discrepancy between training and test distributions, a limitation that VREx~\cite{ahuja2021invariance} addresses by minimizing this variance to improve robustness against extreme distributional shifts and enhance performance in mixed causal and non-causal settings.
Lastly, IRM also needs help in ensuring sufficient invariant predictive factors, as it may inadequately capture robust features within each domain, leading to a reliance on non-invariant, environment-specific factors that harm generalization. 
IB-IRM~\cite{rosenfeld2020risks} tackles this by compressing the entropy of the feature extractor through the information bottleneck method, thus minimizing reliance on environment-specific features and improving invariant prediction. 

\subsection{Data Augmentation}
Other DG methods increase dataset diversity through DA~\cite{yan2020improve, zhang_domain_2024}.
Mixup~\cite{zhang2017mixup} generated new data by mixing two samples, and the Mixup series method has been widely used for domain generalization~\cite{lee_decompose_2023, zhou2021domain}.
For example, MixStyle~\cite{zhou2021domain} generates new domain style samples by mixing the styles between different domains.
Lee \etal~\cite{lee_decompose_2023} applied the Mixup technique in the frequency domain to augment the shape features.
However, these methods still have limitations in that mixing images from two classes does not necessarily result in enhanced samples belonging to them~\cite{concutmix}.

\subsection{Semantic Data Augmentation}
Recent work has introduced Semantic Data Augmentation (SDA), also known as feature augmentation, which applies semantic transformations to features such as background or foreground textures to increase diversity while maintaining computational efficiency~\cite{li_simple_nodate, wang2024inter}. 
For example, Li et al.\cite{li_simple_nodate} proposed adding Gaussian noise to feature embeddings during training to enhance domain generalization. In contrast, Wang et al.\cite{wang2024inter} introduced an SDA-based method to improve diversity across both intra-class and inter-domain variations.
These approaches leverage the typically linear nature of deep features~\cite{bengio2013better, upchurch2017deep}. 
However, like Mixup-based techniques, SDA needs help with label consistency due to over-augmentation, potentially leading to misalignment between the generated features and their original labels~\cite{zhu2024bayesian}. 
To address this, BSDA incorporates variational inference to control semantic transformations and ensure label consistency. 
Despite its success in medical image classification, the broader applicability of BSDA for natural image classification and domain generalization still needs to be explored.

\subsection{Vicinal Risk Minimization}
VRM~\cite{chapelle2000vicinal} is a framework that seeks to improve generalization by minimizing the risk over the distribution of perturbed, yet similar, data points drawn from the original training data. 
Mixup~\cite{zhang2017mixup} and its variants~\cite{zhou2021domain, lee_decompose_2023} techniques are implementations of VRM, as they generate new samples by applying transformations to the training data, effectively increasing the diversity of the dataset and enhancing model robustness. 
Similarly, SDA~\cite{ISDA} can be viewed as a form of VRM, where feature-level semantic transformations are applied to the data, increasing intra-class and inter-domain diversity~\cite{wang2024inter}.

